Online Dynamic Trajectory Optimization and Control for a Quadruped Robot

Legged robot locomotion requires the planning of stable reference trajectories, especially while traversing uneven terrain. The proposed trajectory optimization framework is capable of generating dynamically stable base and footstep trajectories for multiple steps. The locomotion task can be defined with contact locations, base motion or both, making the algorithm suitable for multiple scenarios (e.g., presence of moving obstacles). The planner uses a simplified momentum-based task space model for the robot dynamics, allowing computation times that are fast enough for online replanning.This fast planning capabilitiy also enables the quadruped to accommodate for drift and environmental changes. The algorithm is tested on simulation and a real robot across multiple scenarios, which includes uneven terrain, stairs and moving obstacles. The results show that the planner is capable of generating stable trajectories in the real robot even when a box of 15 cm height is placed in front of its path at the last moment.

==> ral_latest/sections/SLQ.tex <==
\section{Constrained Sequential Linear Quadratic Programming}
We formulate trajectory optimization as a nonlinear optimal control problem as follows,
\begin{equation}
\begin{split}
\label{eqn:OptConProblem}
{\min_{\mathrm{x,u}}} \quad &  {\phi(\mathrm{x}_{t_{f}})}+\sum_{t_{0}}^{t_{f}}{L_i(\mathrm{x,u},t)}\\
\mathrm{s.t.} \quad& \dot{\mathrm{x}}=f_{i}(\mathrm{x,u}),\\
&g_{i}(\mathrm{x,u},t)=0,\;h_{i}(\mathrm{x,u},t)\geq 0,\\
&\mathrm{x} \in \mathcal{X},\; \mathrm{u} \in \mathcal{U}
\end{split}
\end{equation}
where $\mathrm{x,u}$ are state and control input vectors respectively, $f_{i}$ is system dynamics, $\phi,L$ are  final and running costs, and $g_{i},h_{i}$ are phase equality and inequality constraints. Details of each variable and constraint equation are given in the section 3 and 4. 

The problem in Eq. (\ref{eqn:OptConProblem}) is solved with SLQ, where system dynamics are linearized around the result of the previous solution and the cost function is quadratically approximated if not already quadratic. The resulting problem is Linear Quadratic in terms of state and input increments $\delta x$, $\delta u$ and is solved sequentially with a constrained QP solver \cite{frison2014high}.
\iffalse
iteratively using Riccati-like backward sweeps.

The convergence performance can be improved by implementing a line search after each iteration. The unconstrained iLQR algorithm can be extended to constrained iLQR using active-set \cite{tassa2014control} and interior-point methods \cite{frison2014high}.
\fi
